Toward Appearance-based Autonomous Landing Site Identification for Multirotor Drones in Unstructured Environments

A remaining challenge in multirotor drone flight is the autonomous identification of viable landing sites in unstructured environments. One approach to solve this problem is to create lightweight, appearance-based terrain classifiers that can segment a drone's RGB images into safe and unsafe regions. However, such classifiers require data sets of images and masks that can be prohibitively expensive to create. We propose a pipeline to automatically generate synthetic data sets to train these classifiers, leveraging modern drones' ability to survey terrain automatically and the ability to automatically calculate landing safety masks from terrain models derived from such surveys. We then train a U-Net on the synthetic data set, test it on real-world data for validation, and demonstrate it on our drone platform in real-time.

==> sections/discussion.tex <==
\begin{itemize}
    \item adding the TPU to the payload was naively ok but caused the drone to refuse to take off once the TPU started making inferences because of a navigational error. This was fixed by shielding the TPU with aluminum foil and shielding the wire with a ferrite choke, but it still seemed to affect the compass slightly, resulting in the camera/gimbal not quite aligning with the drone in the yaw dimension.
    \item problematic validation cases -- limitations of appearance-based traversability methods
\end{itemize}
